Toward Automated Algorithm Design: A Survey and Practical Guide to Meta-Black-Box-Optimization

In this survey, we introduce Meta-Black-Box-Optimization~(MetaBBO) as an emerging avenue within the Evolutionary Computation~(EC) community, which incorporates Meta-learning approaches to assist automated algorithm design. Despite the success of MetaBBO, the current literature provides insufficient summaries of its key aspects and lacks practical guidance for implementation. To bridge this gap, we offer a comprehensive review of recent advances in MetaBBO, providing an in-depth examination of its key developments. We begin with a unified definition of the MetaBBO paradigm, followed by a systematic taxonomy of various algorithm design tasks, including algorithm selection, algorithm configuration, solution manipulation, and algorithm generation. Further, we conceptually summarize different learning methodologies behind current MetaBBO works, including reinforcement learning, supervised learning, neuroevolution, and in-context learning with Large Language Models. A comprehensive evaluation of the latest representative MetaBBO methods is then carried out, alongside an experimental analysis of their optimization performance, computational efficiency, and generalization ability. Based on the evaluation results, we meticulously identify a set of core designs that enhance the generalization and learning effectiveness of MetaBBO. Finally, we outline the vision for the field by providing insight into the latest trends and potential future directions. Relevant literature will be continuously collected and updated at https://github.com/MetaEvo/Awesome-MetaBBO.

==> table-metabbo-rl.tex <==

\begin{table*}[t]
    \centering
    \caption{Recent publications in MetaBBO-RL, we present their references, publication years, inside RL techniques, adopted neural network architectures and problem set used for training/testing. }
    \label{metabbo-rl}
    \scalebox{0.7}{  % Scale the table to fit within a page column
    \begin{tabular}{c|c|c|c|c|c}
    \hline
    & \textbf{Algorithm} & \textbf{Year} & \textbf{RL} & \textbf{Network} & \textbf{Training/testing set} \\ \hline
    \multirow{37}{*}{\begin{sideways}Value-based method\end{sideways}} 
    & RLMPSO \cite{samma2016rlmpso} & 2016 & Tabular Q-learning \cite{1992qlearning} & — & 10 optimization problems designed by experts and CEC 2005 \\ \cline{2-6}
    & RL-MOEA/D \cite{ning2018rlmoea}& 2018 & SARSA \cite{sutton2018reinforcement} & — & CEC 2009 \\ \cline{2-6}
    & QFA \cite{2018QFA}& 2018 & Tabular Q-learning & — & CEC 2015 \\ \cline{2-6}
    & DE-DDQN \cite{2019deddqn}& 2019 & DDQN \cite{2016ddqn} & MLP & CEC 2005 \\ \cline{2-6}
    & DE-RLFR \cite{2019derlfr}& 2019 & Tabular Q-learning & — & 11 optimization problems designed by experts \\ \cline{2-6}
    & QLMOPSO \cite{liu2019qlmopso}& 2019 & Tabular Q-learning & — & 5 multi-objective functions from ZDT \\ \cline{2-6}
    & QLPSO \cite{2020qlpso}& 2020 & Tabular Q-learning & — & CEC 2013 \\ \cline{2-6}
    & MARLwCMA \cite{sallam2020marlwcma}& 2020 & Tabular Q-learning & — & Problems collected from CEC2011, CEC 2013, CEC 2014, CEC 2015 and CEC 2017 \\ \cline{2-6}
    & LRMODE \cite{huang2020lrmode}& 2020 & Tabular Q-learning & — & ZDT and DTLZ \\ \cline{2-6}
    & RLEA-SSC \cite{xia2021rlea-ssc}& 2021 & Tabular Q-learning & — & 11 problems from the CEC 2013 MMOP \\ \cline{2-6}
    & qlDE \cite{huynh2021qlde}& 2021 & Tabular Q-learning & — & 5 optimization problems designed by experts \\ \cline{2-6}
    & RLDE \cite{hu2021rlde}& 2021 & Tabular Q-learning & — & Single diode model, double diode model, and PV module models \\ \cline{2-6}
    & MADAC \cite{xue2022madac}& 2022 & VDN \cite{sunehag2017vdn} & MLP & DTLZ2, DTLZ4, WFG4, and WFG9 \\ \cline{2-6}
    & MOEA/D-DQN \cite{tian2022modead-dqn}& 2022 & DDQN & MLP & ZDT, DTLZ, WFG, and UF \\ \cline{2-6}
    & ALDES \cite{zhao2024aldes}& 2022 & - & - & PBO and real-world problems \\ \cline{2-6}
    & RL-CORCO \cite{hu2022rl-corco}& 2022 & Tabular Q-learning & — & CEC 2010 and CEC 2017 \\ \cline{2-6}
    & RL-SHADE \cite{2022rlshade}& 2022 & Tabular Q-learning & — & CEC special sessions on real-parameter single-objective optimization \\ \cline{2-6}
    & RLLPSO \cite{wang2022rllpso}& 2022 & Tabular Q-learning & — & CEC 2010 LSGO and CEC 2013 LSGO \\ \cline{2-6}
    & RL-HPSDE \cite{2022rlhpsde}& 2022 & Tabular Q-learning & — & CEC 2017 \\ \cline{2-6}
    & MARLABC \cite{zhao2023marlabc}& 2023 & Tabular Q-learning & — & CEC 2017 \\ \cline{2-6}
    & RLHDE \cite{peng2023rlhde}& 2023 & Tabular Q-learning & — & 7 global trajectory optimization problems on GTOP \\ \cline{2-6}
    & Q-LSHADE \cite{qlshade}& 2023 & Tabular Q-learning & — & CEC 2018 \\ \cline{2-6}
    & RLMMDE \cite{han2023rlmmde}& 2023 & Tabular Q-learning & — & ZDT, DTLZ, and UF \\ \cline{2-6}
    & RLDMDE \cite{yang2024rldmde}& 2023 & Tabular Q-learning & — & CEC 2013 and CEC 2017 \\ \cline{2-6}
    & MPSORL \cite{meng2023mpsorl}& 2023 & Tabular Q-learning & — & CEC 2017 and CEC 2019 \\ \cline{2-6}
    & NRLPSO \cite{li2023nrlpso}& 2023 & Tabular Q-learning & — & CEC 2017 \\ \cline{2-6}
    & DQ-HSES \cite{qlshade}& 2023 & DQN & MLP & CEC 2018 \\ \cline{2-6}
    & DE-DQN \cite{2021dedqn} & 2023 & DQN & MLP & CEC 2017 \\ \cline{2-6}
    & CEDE-DRL \cite{hu2023cede-drl}& 2023 & DQN & MLP & CEC 2010 and CEC 2017 \\ \cline{2-6}
    & SA-DQN-DE \cite{liao2024sa-dqn-de}& 2023 & DQN & MLP & CEC 2013 \\ \cline{2-6}
    & UES-CMAES-RL \cite{2024uescmaesrl}& 2024 & DQN & MLP & CEC 2013 \\ \cline{2-6}
    & R2-RLMOEA \cite{tahernezhad2024r2-rlmoea}& 2024 & DDQN & MLP & CEC 2009 \\ \cline{2-6}
    & RLNS \cite{2024PSORLNS}& 2024 & Tabular Q-learning & — & CEC 2015 multi-niche benchmark \\ \cline{2-6}
    & RLMODE \cite{yu2024rlmode}& 2024 & Tabular Q-learning & — & 30 optimization functions designed by experts \\ \cline{2-6}
    & MRL-MOEA \cite{wang2024mrl-moea}& 2024 & Tabular Q-learning & — & DTLZ and WFG \\ \cline{2-6}
    & MSoRL \cite{wang2024msorl}& 2024 & Tabular Q-learning & — & CEC 2010 LSGO and CEC 2013 LSGO \\ \cline{2-6}
    & HHRL-MAR \cite{as-add-6}& 2024 & Tabular Q-learning & — & CEC 2017 and CEC 2020 \\ \cline{2-6}
    & HF \cite{pei2024learning}& 2024 & DDQN & MLP & CEC 2005, CEC 2017 and CVRPTW \\ \hline
    
    \multirow{15}{*}{\begin{sideways}Policy gradient\end{sideways}} 
    & LTO \cite{shala2020lto}& 2020 & GPS \cite{levine2013gps} & LSTM & The COCO platform, and HPO \\ \cline{2-6}
    & RLEPSO \cite{yin2021rlepso}& 2021 & DDPG \cite{silver2014ddpg}& MLP & Shifted and rotated CEC 2013 \\ \cline{2-6}
    & LDE \cite{sun2021lde}& 2021 & REINFORCE \cite{1992REINFORCE} & LSTM & CEC 2013 \\ \cline{2-6}
    & RL-PSO \cite{wu2022rl-pso} & 2022 & REINFORCE & MLP & CEC 2015 learning-based suite \\ \cline{2-6}
    & REM \cite{zhang2022rem}& 2022 & REINFORCE & — & CEC 2018 \\ \cline{2-6}
    & MELBA \cite{chaybouti2022melba}& 2022 & PPO & Transformer & PROFET \\ \cline{2-6}
    & MOEADRL \cite{gao2023moeadrl}& 2023 & A2C \cite{1999Actor-critic} & — & SMOP \\ \cline{2-6}
    & LADE \cite{liu2023lade}& 2023 & REINFORCE & LSTM & CEC 2013 \\ \cline{2-6}
    & RLAM \cite{2023rlam}& 2023 & DDPG & MLP & CEC 2013 \\ \cline{2-6}
    & AMODE-DRL \cite{li2023amode-drl}& 2023 & DDQN + DDPG & MLP & Practical problems and randomly generated problems \\ \cline{2-6}
    & PG-DE \cite{zhang2024pg-de}& 2024 & REINFORCE & MLP & CEC 2018 \\ \cline{2-6}
    & GLEET \cite{ma2024gleet}& 2024 & PPO & MLP and Transformer & Augmented CEC 2021 \\ \cline{2-6}
    & RLEMMO \cite{lian2024rlemmo}& 2024 & PPO & MLP and Transformer & CEC 2013 MMOP \\ \cline{2-6}
    & RL-DAS \cite{2024rldas}& 2024 & PPO & MLP & CEC 2021 \\ \cline{2-6}
    & SYMBOL \cite{2024symbol}& 2024 & PPO & LSTM & 10 challenging synthetic BBO problems from CEC 2021 \\ \hline
    \end{tabular}
    }
\end{table*}

